Sampled Transformer for Point Sets

The sparse transformer can reduce the computational complexity of the self-attention layers to $O(n)$, whilst still being a universal approximator of continuous sequence-to-sequence functions. However, this permutation variant operation is not appropriate for direct application to sets. In this paper, we proposed an $O(n)$ complexity sampled transformer that can process point set elements directly without any additional inductive bias. Our sampled transformer introduces random element sampling, which randomly splits point sets into subsets, followed by applying a shared Hamiltonian self-attention mechanism to each subset. The overall attention mechanism can be viewed as a Hamiltonian cycle in the complete attention graph, and the permutation of point set elements is equivalent to randomly sampling Hamiltonian cycles. This mechanism implements a Monte Carlo simulation of the $O(n^2)$ dense attention connections. We show that it is a universal approximator for continuous set-to-set functions. Experimental results on point-clouds show comparable or better accuracy with significantly reduced computational complexity compared to the dense transformer or alternative sparse attention schemes.

==> additional_single_layer.tex <==
%!TEX root = ../iclr2023_conference.tex
\begin{table}[t]
    \caption{Additional object classification accuracy (\%) for different attention mechanisms in the basic setting.
    OM denotes \textit{out of memory}.}%
    \label{tab:additional_single_layer}%
    \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|cccccccc}
            \toprule
            \#Points & 256 & 512 & 768 & 1024 & 2048 & 3072 & 4096 & 8192 \\
            \midrule
            MLP + FC (no attention) & 85.96 & 86.24 & 85.43 & 85.96 & 85.84 & 86.61 & 86.32  & 86.13 \\
            Inducting Points \citep{lee2019set} & 84.21 & 81.25 & 82.55 & 81.57 & 80.96 & 76.18 & 75.13 & 75.65 \\
            Stratified Strategy \citep{lai2022stratified} & 87.21 & 87.62 & 86.69 & 85.99 & 85.34 & 84.32 & OM & OM \\
            Sampled Attention & \textbf{87.34} & \textbf{87.93} & \textbf{87.66} & \textbf{88.03} & \textbf{87.82} & \textbf{87.18} & \textbf{87.46} & \textbf{87.73} \\
            \bottomrule
        \end{tabular}
        }
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,pifont,nicefrac}
\usepackage{mathrsfs}
\usepackage{csquotes}

% ---- Alex commands ----
\newcommand{\todo}[1]{{\color{red} \textbf{#1}}}

\newcommand{\defeq}{\doteq}

% Sparse attention
\newcommand{\shead}{\text{SHead}}
\newcommand{\sattn}{\text{SAttn}}
\newcommand{\stb}{\text{STB}}

%\newcommand{\subX}{\overline{\bm \mathsf{X}}}
\newcommand{\subX}{{\bm {\mathsf{X}}}}
%\newcommand{\uppert}{\mathrm{up}}
%\newcommand{\lowert}{\mathrm{low}}
\newcommand{\uppert}{\uparrow}
\newcommand{\lowert}{\downarrow}

\newcommand{\shiftop}{S}
\newcommand{\shiftu}{\shiftop^{\uppert}}
\newcommand{\shiftl}{\shiftop^{\lowert}}
\newcommand{\bmshiftu}{{\bm\shiftop}^{\uppert}}
\newcommand{\bmshiftl}{{\bm\shiftop}^{\lowert}}

\newcommand{\indicator}{\mathbb{1}}
\newcommand{\zeros}{\mathbb{0}}
\newcommand{\pow}{\mathcal{P}} % Powerset

\newcommand{\U}{{\mathsf{U}}}
\newcommand{\V}{{\mathsf{V}}}
% ---- Alex commands ----

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\usepackage{bbold}

==> sparse_tf.tex <==

\subsection{Sparse Transformer and Universal Approximator}
Similar to Eq.~\ref{eq:dense_tf} the sparse transformer is definited as:
\begin{subequations}
   \begin{align}
      &\text{SAttn}^l(\bm X) = \bm X + \bm W_O \begin{bmatrix} \text{SHead}^{1,l}(\bm X) \\ \vdots \\ \text{SHead}^{h,l}(\bm X) \end{bmatrix}\\
      &\text{SHead}^{i,l}(\bm X)_k = \bm W^i_V \bm X_{\mathcal{A}^l_k} \cdot \sigma_S [ (\bm W^i_K \bm X_{\mathcal{A}^l_k})^T \bm W^i_Q \bm X_k] \\
      &\text{STB}(\bm X) = \text{SAttn}^l(\bm X) + \bm W_2 \cdot \text{ReLU}(\bm W_1 \text{SAttn}^l(\bm X)),
   \end{align}
   \label{eq:sparse_tf}
\end{subequations}
here $\mathcal{A}^l_k$, for $l\in [p]$ and $k\in [n]$, is the $l$-th sparsity pattern on $k$-th column (token embedding).
$\bm X_{\mathcal{A}^l_k} \in \mathbb{R}^{d\times m}$ is the set of token embeddings 'links' to $k$-th token embedding under $l$-th sparse partten.
\begin{definition}
   The sparsity patterns $\{ \mathcal{A}^l_k \}$ satisfy the following:
   \begin{enumerate}
      \item For all $k\in [n]$ and $l\in [p]$, we have $k \in \mathcal{A}^l_k$.
      \item There exists a permutation $\gamma: [n] \to [n]$ such that, for all $i \in [n-1]$, $\gamma(i) \in \cup^p_{l=1}\mathcal{A}^l_{\gamma(i+1)}$.
      \item There exists a finite $s \in \mathbb{N}$ such that $s = \min\{ u \vert  \mathcal{S}^u_k = [n] \text{ for all } k \in [n] \}$.
   \end{enumerate}
\end{definition}
The first rule means each sparse pattern should include itself. The second says there exist a perumation such that the sparse attention of the current token embedding includes the previous one.
The last rule says after $s$ sparse attention layers, every token are directly or indirectly linked to all others.

The proof of universal approximator for sparse transformer is same to the dense transformer except proofing contextual mapping, as all other steps only require using feed-forward layers.
So the key point is proofing the sparse multi-head attention is contextual mapping.
Difference with dense multi-head attention, the sparse one could not visit the all tokens in one step, so could not apply the selective shift operation directly.
In fact it requires $\delta^{-nk}$ number of sparase multi-head attentions rather than $\delta^{-k}$ in the dense case.

The sparse multi-head attention is implemented as:
\begin{subequations}
   \begin{align}
      &\Psi^l(\bm Z; c, b_Q, b'_Q) := \bm Z + [c\bm e^{(1)} -c\bm e^{(1)}] 
      \begin{bmatrix}
         \psi^l (\bm Z; b_Q) \\
         \psi^l (\bm Z; b'_Q)
      \end{bmatrix}\\
      &\psi^l(\bm Z; b_Q)_k := \bm u^T \bm Z_{\mathcal{A}^l_k} \sigma_H [(\bm u^T \bm Z_{\mathcal{A}^l_k})^T(\bm u^T \bm Z_k - b_Q)]=
      \begin{cases}
         \max_{j\in \mathcal{A}^l_k}\bm u^T \bm Z_j & \text{if } \bm u^T \bm Z_k > b_Q,\\
         \min_{j\in \mathcal{A}^l_k}\bm u^T \bm Z_j & \text{if } \bm u^T \bm Z_k < b_Q.
      \end{cases}
   \end{align}
\end{subequations}
Compared with Eq.~\ref{eq:selective_shift}, the sparse selective shift operation only takes the maximum and minimum w.r.t $\mathcal{A}^l_k$ rather than all tokens.
The $(1, k)$-th entry reads
\begin{subequations}
\begin{align}
   \Psi^l (\bm Z; c, b_Q, b'_Q)_{1,k} &= Z_{1,k} + c\left(\psi^l (\bm Z; b_Q)_k - \psi^l (\bm Z; b'_Q)_k \right)\\
   &= 
   \begin{cases}
      Z_{1,k} + c\left( \max_{j\in \mathcal{A}^l_k} \bm u^T \bm Z_j - \min_{j\in \mathcal{A}^l_k} \bm u^T \bm Z_j  \right) & \text{if } b_Q < \bm u^T \bm Z_k < b'_Q,\\
      Z_{1,k} & \text{if } \bm u^T\bm Z_k \notin [b_Q, b'_Q].
   \end{cases}
\end{align}
\end{subequations}
Same as in Eq.~\ref{eq:selective_shift_col}, the sparse shift operation only modify each entries in the first row of the input $\bm Z_{1,k}$ if $\bm u^T \bm Z_k \in (b_Q, b'_Q)$, which is also an one-to-one mapping.

However, as the sparse attention could not reach a subset of tokens, the global maximum and minimum could not be calculated in general cases.
This could be solved by assuming $l_2 < l_3 < \cdots < l_n < l_1$, which is achieved by the positional embedding
\begin{align}\label{eq:position_embedding}
   \bm E = 
   \begin{bmatrix}
      n - 1 & \cdots & n - 1\\
      i - 2 & \cdots & i - 2\\
      i - 3 & \cdots & i - 3\\
      \cdots & \cdots & \cdots \\
      n - 2 & \cdots & n - 2
   \end{bmatrix}.
\end{align}
Rewrite the input space from $\mathbb{G}_\delta$ to
\begin{align}
   \mathbb{H}_\delta := \{ \bm G + \bm E \in \mathbb{R}^{d\times n} \vert \bm G \in \mathbb{G}_\delta := [0, \delta, 1-\delta]^{d\times n} \}.
\end{align}
And the interval will be
\begin{align}
   &\bm H_1 \in [n-1:\delta:n-\delta]^d,\\
   &\bm H_i \in [i-2:\delta:i-1-\delta]^d \text{ for all } i \in [2:n].
\end{align}
By choicing $\bm u := (1, \delta^{-1}, \delta^{-2}, \dotso, \delta^{-d+1})$, the map $\bm H_k \mapsto \bm u^T \bm H_k$ is one-to-one, and
\begin{align}\label{eq:pe_interval}
   &\bm u^T \bm H_{1} \in \left[ (n-1)\sum_{i=0}^{d-1} \delta^{-i}: \delta: (n-1)\sum_{i=0}^{d-1} \delta^{-i} + \delta^{-d+1} - \delta \right],\\
   &\bm u^T \bm H_{i} \in \left[ (i-2)\sum_{i=0}^{d-1} \delta^{-i}: \delta: (i-2)\sum_{i=0}^{d-1} \delta^{-i} + \delta^{-d+1} - \delta \right] \text{ for all } i \in [2:n].
\end{align}
So the interval of the dot product $\bm u^T \bm H_i$ is disjoint and $\bm u^T \bm H_2 < \bm u^T \bm H_3 < \cdots < \bm u^T \bm H_n < \bm u^T \bm H_1$.
As the $j$-th token is linked to itself and the previous one, we could calculate the maximum and minimum value in selective shift operation:
The sparase selective shift operation is first applied to second column, which is the minimum one, and its previous token (first column) is the maximum one.
After this step, the resulted $\bm u^T \tilde{\bm H}_2$ is the new maximum and the thrid column $\bm u^T \bm H_3$ is the new minimum one.
And the next sparsed selective shift operation could be applied to $\bm u^T \bm H_3$ as the maximum and minimum is reached by $\mathcal{A}^l_3$.
After $n-1$ steps of sparse selective shift operations, we have $\bm u^T \bm H_1 < \bm u^T \tilde{\bm H}_2 < \bm u^T \tilde{\bm H}_3 \cdots < \bm u^T \tilde{\bm H}_n$.
This operation could guarantee the first rule of contextual mapping.

Then the all-max shift operation is applied to guarantee that all 'column ids' for different input (contextual) is disjoint, so the second rule of the contextual mapping is implemented.
The all-max shift operation $\Omega^l : \mathbb{R}^{d\times n} \to \mathbb{R}^{d\times n}$ is defined as
\begin{align}
   \Omega^l (\bm Z; c) = \bm Z + c\bm e^{(1)}\psi^l (\bm Z; 0).
\end{align}
And the $(1, k)$-th entry reads
\begin{align}
   \Omega^l (\bm Z; c)_{1,k} = Z_{1,k} + c \psi^l (\bm Z; 0)_k = Z_{1,k} + c \max_{j \in \mathcal{A}^l_k} \bm u^T \bm Z_j.
\end{align}
To reach the global maximum, at least $s$ all-max shift operations should be applied.
The total number of multi-head attention layers is $\delta^{-nk}+s$.

\section{Masked Transformer}
The masked transformer is defined as masking some tokens and replacing it with shared learnable masking token embedding $\bm m \in \mathbb{R}^d$, and $\bm M = [\bm m^T, \dotso, \bm m^T] \in \mathbb{R}^{d\times n}$.
The randomly masking indicator is defined as $\bm \xi_n \in \{ 0, 1\}^n$ with 0 indicates the masked token.
And $\circ$ denotes Hadamard product.
\begin{subequations}
   \begin{align}
      &\text{Mask}(\bm X, \bm M) = \bm X \circ (\bm 1_d^T \bm \xi_n) + \bm M \circ \left( \bm 1_d^T (\bm 1_n - \bm \xi_n) \right) \\
      &\text{SHead}^{i,l}(\bm X)_k = \bm W^i_V \text{Mask}(\bm X)_{\mathcal{A}_k^l} \cdot \sigma_S [ (\bm W^i_K \text{Mask}(\bm X)_{\mathcal{A}_k^l})^T \bm W^i_Q \text{Mask}(\bm X)_k] \\
      &\text{SAttn}^l(\bm X) = \bm X + \bm W_O \begin{bmatrix} \text{SHead}^{1,l}(\bm X) \\ \vdots \\ \text{SHead}^{h,l}(\bm X) \end{bmatrix}\\
      &\text{STB}^l(\bm X) = \text{SAttn}^l(\bm X) + \bm W_2 \cdot \text{ReLU}(\bm W_1 \cdot \text{SAttn}^l(\bm X)).
   \end{align}
   \label{eq:masked_tf}
\end{subequations}

